TTR-Based Reward for Reinforcement Learning with Implicit Model Priors

Model-free reinforcement learning (RL) is a powerful approach for learning control policies directly from high-dimensional state and observation. However, it tends to be data-inefficient, which is especially costly in robotic learning tasks. On the other hand, optimal control does not require data if the system model is known, but cannot scale to models with high-dimensional states and observations. To exploit benefits of both model-free RL and optimal control, we propose time-to-reach-based (TTR-based) reward shaping, an optimal control-inspired technique to alleviate data inefficiency while retaining advantages of model-free RL. This is achieved by summarizing key system model information using a TTR function to greatly speed up the RL process, as shown in our simulation results. The TTR function is defined as the minimum time required to move from any state to the goal under assumed system dynamics constraints. Since the TTR function is computationally intractable for systems with high-dimensional states, we compute it for approximate, lower-dimensional system models that still captures key dynamic behaviors. Our approach can be flexibly and easily incorporated into any model-free RL algorithm without altering the original algorithm structure, and is compatible with any other techniques that may facilitate the RL process. We evaluate our approach on two representative robotic learning tasks and three well-known model-free RL algorithms, and show significant improvements in data efficiency and performance.

==> related_work.tex <==
\section{RELATED WORK}

Recently, deep neural network has been prevailing in RL in different areas such as games, robotics and natural language processing \cite{c17, c18, c19}. The deep Q-network (DQN) \cite{c20} was developed to learn directly from image pixels to play 2600 Atari video games at a superhuman level. It provides solutions for instability of function approximation techniques in the class of value-based RL method. Deep Deterministic Policy Gradient (DDPG) \cite{c45} features at concurrently learning Q-value function and upgrades DQN in continuous state and action space. Policy-based methods, including Vanilla Policy Gradient \cite{c46, c47}, Trust Region Policy Optimization (TRPO) \cite{c22} and Proximal Policy Optimization (PPO) \cite{c23} aims to find policies directly by means of gradient-based method. In our work, DDPG, TRPO and PPO are selected as three novel model-free optimization algorithms to test the performance of TTR-based reward.


Substantial data inefficiency still remains as a major challenge in solving RL problem \cite{c1}. Various techniques have been proposed to address it. "Deep exploration" \cite{c1} strategy alleviates this problem by maintaining a distribution over possible values and bootstrapping from it with random initialization. Count-based exploration \cite{c40} is dedicated to extending the near-optimal count-based exploration algorithms into high-dimensional state space. Curriculum-based approaches \cite{c03} paved another possible way to overcome data inefficiency by learning progressively over multiple sub-problems with different difficulty level. The training starts on easier sub-problems and gradually transits to much harder sub-problems until the original full problem becomes appropriate to train on directly. Hierarchical RL framework \cite{c3,c4,c5} tries to improve data efficiency by building modules with different levels, in which top-level module learns a policy over options (sub-goals) and the bottom-level module learns policies to accomplish the objective of each option.

The TTR-based reward shaping method proposed in this work attributes to the topic of reward shaping, a classic technique that provides additional localized feedback based on prior knowledge to guide the learning process \cite{c6}. Reward shaping has been proven to be a simple but powerful method for reducing sample complexity and speed up RL tasks. Randlov and Alstrom \cite{c7} first use shaping function to learn control policy for bicycle navigation . However, the function requires strenuous engineering labour to hand-tune. Ng, Harada, and Russell \cite{c9} raised up potential-based reward shaping (PBRS), proving the conditions that an arbitrary externally specified reward shaping function must satisfy if they could be included in a RL system without modifying its optimal policy. Based on PBRS, Wiewiora \cite{c10} proposed the potential-based advice (PBA) framework that allows the potential function to also include actions while still restricted with PBRS conditions. Furthermore, Inverse Reinforcement Learning (IRL) technique arises as an distinct perspective to learn a reward function directly from the expert demonstrations, thereby avoiding the manual specification \cite{c11, c12}. 

Recently, incorporating prior model knowledge into model-free learning acquires more research attention. Boris \cite{c16} apply system dynamics as prior knowledge for stable curricula generation to accelerate learning process. Ofir \cite{c15} allow the full transition information as prior beliefs to provide shaping reward directly without learning through interactions with environment. Our work is inspired by the high-level idea of utilizing system dynamics to improve data efficiency of model-free RL. Specifically, we leverage model dynamics as prior to offer shaped reward directly without any engineering labour or interactions with environment.

TTR problem is an important class of optimal control problems. It includes finding the minimum time that takes a system to reach certain goal region starting from any initial state under particular system constraints. The common approach for tackling TTR problems is to solve a Hamilton-Jacobi (HJ) partial differential equation (PDE) corresponding to system dynamics and this approach is widely applicable to both continuous and hybrid systems \cite{c25, c26, c27}. Normally the computational cost of solving TTR problem is too expensive for system with high-dimensional state. However, model simplification and system decomposition techniques make a significant leap in alleviating the computational burden in a variety of problem setups \cite{c28, c29}. It is proved by various tests \cite{c30} that approximating the TTR by simplifying  model dynamics or applying system decomposition is feasible and computational efficiently .  
